Aerial Robot Control in Close Proximity to Ceiling: A Force Estimation-based Nonlinear MPC

Being motivated by ceiling inspection applications via unmanned aerial vehicles (UAVs) which require close proximity flight to surfaces, a systematic control approach enabling safe and accurate close proximity flight is proposed in this work. There are two main challenges for close proximity flights: (i) the trust characteristics varies drastically for the different distance from the ceiling which results in a complex nonlinear dynamics; (ii) the system needs to consider physical and environmental constraints to safely fly in close proximity. To address these challenges, a novel framework consisting of a constrained optimization-based force estimation and an optimization-based nonlinear controller is proposed. Experimental results illustrate that the performance of the proposed control approach can stabilize UAV down to 1 cm distance to the ceiling. Furthermore, we report that the UAV consumes up to 12.5% less power when it is operated 1 cm distance to ceiling, which is promising potential for more battery-efficient inspection flights.

==> Abstract/00_Abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
This paper describes a systematic approach for aerial robots able to fly in close proximities which can perform various tasks including ceiling inspection. This work is motivated by the exploration of efficient flight for such systems to interact with the surroundings. However, these applications may bring additional challenges, i.e., (i) the thrust coefficient increases while it approaches the ceiling, which eliminates the linearity assumption for the control allocation matrix; (ii) the thrust efficiency changes in different proximities to the ceiling which may not result in a required counter force generation; (iii) the system needs to consider physical and environmental constraints to safely fly in close proximities. To address these challenges, a novel framework consisting of a constrained optimization-based force estimation and an optimization-based controller is proposed. Experimental results illustrate the effectiveness of the proposed approach and the promising potential in terms of more efficient flight, where the current drawn from the battery is decreased ($\approx$15.8) while it flies below 1 cm from the ceiling.
\end{abstract}
%\begin{IEEEkeywords}
%Piezoceramic materials, energy harvesting, electromagnetic induction, UAV
%\end{IEEEkeywords}

==> Sections/4_Num_Inves.tex <==


%In the flight tests, the flying robot first reached a random point. After this hovering phase, a reference is generated to go below the ceiling. In order to evaluate system performance, different proximities are defined. In the first experiment, the system needs to hover by keeping its orientation below 16 cm from the ceiling. In Fig. \ref{ceiling16}, the system response on the tracking (Fig. \ref{fig_z_16}), controller action (Fig. \ref{fig_c_16}) and the force estimation (Fig. \ref{fig_f_16}) can be seen. The first instant of the green region indicates the switching mechanism, where the force estimation-based NMPC is activated. In the first part of the figures, the nominal model-based NMPC is used. As can be seen, the controller can bring the system to the defined reference when the additive model is leveraged. 

%\begin{figure*}[htp]
%	\subfloat[The system performance on vertical axis]
%	{
%		\includegraphics[width=2.3in]{Figures/z16}
%		\label{fig_z_16}
%	} 
%	\subfloat[Control effort]
%	{
%		\includegraphics[width=2.3in]{Figures/controller16}
%		\label{fig_c_16}
%	} 
%	\subfloat[Force estimation]
%	{
%		\includegraphics[width=2.3in]{Figures/estforce16}
%		\label{fig_f_16}
%	}
%	\caption{The system performance below 16 cm}
%	\label{ceiling16}	
%\end{figure*}

%Similar to the first case, the system is also tested below 11 cm from the ceiling. When the switching mechanism is activated, the proposed approach actively suppress the ceiling effect. It is noted that the disturbance on the system becomes more dominant while it flies within 10 cm range as can be seen from Fig. \ref{ceiling11}. 

%\begin{figure*}[htp]
%	\subfloat[The system performance on vertical axis]
%	{
%		\includegraphics[width=2.3in]{Figures/z11}
%		\label{fig_z_11}
%	} 
%	\subfloat[Control effort]
%	{
%		\includegraphics[width=2.3in]{Figures/controller11}
%		\label{fig_c_11}
%	} 
%	\subfloat[Force estimation]
%	{
%		\includegraphics[width=2.3in]{Figures/estforce11}
%\label{fig_f_11}
%	}
%	\caption{The system performance below 11 cm}
%	\label{ceiling11}	
%\end{figure*}

%The system performance below 6 cm from the ceiling is given in Fig. \ref{ceiling6}. The active force estimation-based NMPC mitigates the ceiling effect. As compared to Fig. \ref{fig_c_16} and Fig. \ref{fig_c_11}, the controller effort is decreased. Since the ceiling effect increases the rotor wake which results in an increase in the thrust; to stay in close proximities to the ceiling, the system does not need to generate the same thrust when hovering in the free flight case

%\begin{figure*}[htp]
%	\subfloat[The system performance on vertical axis]
%	{
%		\includegraphics[width=2.3in]{Figures/z06}
%		\label{fig_z_6}
%	} 
%	\subfloat[Control effort]
%	{
%		\includegraphics[width=2.3in]{Figures/controller06}
%		\label{fig_c_6}
%	} 
%	\subfloat[Force estimation]
%	{
%		\includegraphics[width=2.3in]{Figures/estforce06}
%		\label{fig_f_6}
%	}
%	\caption{The system performance below 6 cm}
%	\label{ceiling6}	
%\end{figure*}

%One of the extreme cases, i.e., staying 1 cm below the ceiling, is tested in this implementation as can be seen in Fig. \ref{ceiling1}. The system still handles the ceiling effect in order not to be in permanent physical contact with the ceiling. Since the battery state is observed online in this implementation, it is explored that the current drawn from the battery can be decreased significantly during the flight in very close proximities. 

%\begin{figure*}[htp]
%	\subfloat[The system performance on vertical axis]
%	{
%		\includegraphics[width=2.3in]{Figures/z01}
%		\label{fig_z_1}
%	} 
%	\subfloat[Control effort]
%	{
%		\includegraphics[width=2.3in]{Figures/controller01}
%		\label{fig_c_1}
%	} 
%	\subfloat[Force estimation]
%	{
%		\includegraphics[width=2.3in]{Figures/estforce01}
%		\label{fig_f_1}
%	}\\
%	\subfloat[Battery state]
%	{
%		\includegraphics[width=2.3in]{Figures/battery01}
%		\label{fig_b_1}
%	}
%	\caption{The system performance below 1 cm}
%	\label{ceiling1}	
%\end{figure*}

%The statistical results are summarized in Fig. \ref{ceilingstat}. The battery current for each distance is also presented in Fig. \ref{batterystat}.

%\begin{figure}[h!]
%	{
%		\includegraphics[width=\columnwidth]{Figures/stat_box_ceiling}
%	} 
%	\caption{The statistical results: ceiling effect in different proximities}
%	\label{ceilingstat}	
%\end{figure}



==> Settings/BBKglossary.tex <==
\newacronym{AC}{AC}{alternating current}
\newacronym{DC}{DC}{direct current}

\newacronym{BESS}{BESS}{battery energy storage system}
\newacronym{BMS}{BMS}{battery management system}
\newacronym{btms}{B-TMS}{battery-TMS}
\newacronym{stms}{S-TMS}{system-TMS}
\newacronym{TMS}{TMS}{thermal management system}


\newacronym{DSO}{DSO}{distribution system pperator}
\newacronym{ISO}{ISO}{independent system operator}
\newacronym{PV}{PV}{photovoltaic}
\newacronym{IoT}{IoT}{Internet of Things}
\newacronym{EOL}{EOL}{end of life}


\newacronym{ESS}{ESS}{energy storage system}
\newacronym{ECM}{ECM}{equivalent circuit model}

\newacronym{EMS}{EMS}{energy management system}
\newacronym{ROI}{ROI}{return on investment}
\newacronym{RES}{RES}{renewable energy source}
\newacronym{pv-bess}{PV-BESS}{residential photovoltaic nattery storage system}
\newacronym{PS}{PS}{peak shaving}

\newacronym{IDM}{IDM}{intraday market}
\newacronym{DAM}{DAM}{day ahead market}
\newacronym{PER}{PER}{power-to-energy ratio}
\newacronym{PCM}{PCM}{Physical-chemical models}
\newacronym{PCR}{PCR}{primary control reserve}
\newacronym{UPS}{UPS}{uninterruptible power supply}
\newacronym{NCA}{NCA}{Nickel-Cobalt-Aluminum-Oxide}
\newacronym{LFP}{LFP}{lithium-iron-phosphate}
\newacronym{NMC}{NMC}{Nickel-Manganese-Cobalt}
\newacronym{LTO}{LTO}{Lithium-Titanate-Oxide}
\newacronym{C}{C}{Carbon-Graphite}
\newacronym{PbA}{PbA}{Lead(Pb)-acid}
\newacronym{NaS}{NaS}{Sodium–sulfur Battery}
\newacronym{TCO}{TCO}{Total Cost of Ownership}
\newacronym{DOF}{DOF}{degrees of freedom}
\newacronym{SOC}{SOC}{state of charge}
\newacronym{SEI}{SEI}{solid electrolyte interphase}
\newacronym{SOH}{SOH}{state of health}
\newacronym{doc}{DOC}{depth of cycle}
\newacronym{DOD}{DOD}{depth of discharge}
\newacronym{OCV}{OCV}{Open Circuit Voltage}
\newacronym{LiS}{LiS}{Lithium-Sulfur}
\newacronym{FEC}{FEC}{full equivalent cycle}
\newacronym{SCADA}{SCADA}{Supervisory Control and Data Acquisition}
\newacronym{DCH}{DCH}{discharge}
\newacronym{CH}{CH}{charge}
\newacronym{MOX}{MO$_{X}$}{Metal-Oxide}

\newacronym{LCOE}{LCOE}{Levelized Cost of Electricity}
\newacronym{MPPT}{MPPT}{Maximum Power Point Tracker}


\newacronym{XHV}{XHV}{Extra-High-Voltage}
\newacronym{HV}{HV}{High-Voltage}
\newacronym{MV}{MV}{Medium-Voltage}
\newacronym{LV}{LV}{Low-Voltage}
\newacronym{BTM}{BTM}{Behind-the-Meter}
\newacronym{MG}{MG}{Micro-Grid}

\newacronym{V2G}{V2G}{Vehicle-to-Grid}
\newacronym{EV}{EV}{Electric Vehicles}

\newacronym{MILP}{MILP}{mixed integer linear programming}
\newacronym{LP}{LP}{linear programming}
\newacronym{NLP}{NLP}{non-linear programming}
\newacronym{DP}{DP}{dynamic programming}

\newacronym{FLC}{FLC}{fuzzy logic}
\newacronym{GA}{GA}{genetic algorithm}
\newacronym{INVM}{INVM}{inventory model}
\newacronym{MPC}{MPC}{model predictive control}
\newacronym{PSO}{PSO}{particle swarm optimisation}


%-----------
\newacronym{PWA}{PWA}{piecewise affine}
\newacronym{EU}{EU}{European Union}

\newacronym[longplural={lithium-ion batteries}]
 {LIB}{LIB}{lithium-ion battery}
 
 %\newacronym{LIB}{LIB}{Lithium-Ion Battery}
